Algorithm and proof as \Omega-invariance and transfer: A new model of computation in nonstandard analysis

We propose a new model of computation based on nonstandard analysis. Intuitively, the role of "algorithm" is played by a new notion of finite procedure, called Omega-invariance and inspired by physics, from nonstandard analysis. Moreover, the role of 'proof' is taken up by the Transfer Principle from nonstandard analysis. We obtain a number of results in Constructive Reverse Mathematics to illustrate the tight correspondence to Errett Bishop's Constructive Analysis and the associated Constructive Reverse Mathematics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{97}
\providecommand{\publicationstatus}{B. L\"owe, G. Winskel (Eds.):\\
Developments in Computational Models 2012 (DCM 2012)\\
EPTCS 143, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.143.9}{10.4204/EPTCS.143.9}}
\pdfoutput=1

